A Framework to Handle Linear Temporal Properties in (\omega-)Regular Model Checking

Since the topic emerged several years ago, work on regular model checking has mostly been devoted to the verification of state reachability and safety properties. Though it was known that linear temporal properties could also be checked within this framework, little has been done about working out the corresponding details. This paper addresses this issue in the context of regular model checking based on the encoding of states by finite or infinite words. It works out the exact constructions to be used in both cases, and proposes a partial solution to the problem resulting from the fact that infinite computations of unbounded configurations might never contain the same configuration twice, thus making cycle detection problematic.

==> expe.tex <==
\section{Experimental Results}
\label{sect-experiments}
				   
The techniques and algorithms presented in this paper have been tested
on several examples covering different classes of systems and
properties. We used T(O)RMC\,\cite{Leg08} to solve the
($\omega$-)regular reachability problems.

First, we considered several examples of parametric networks
corresponding to mutual exclusion protocols including the Bakery
algorithm and the token ring protocol. For these systems, we have been
able to check mutual exclusion properties.

Next, we have been able to check termination or non-termination of
(multi-loop) programs manipulating integer variables.

Finally, we also addressed the problem of verifying a liveness property of
a system manipulating counters as well as (continuous time)
clocks. One of the examples we considered is a simplified model of the
IEEE~1394 root contention protocol, which is described in
\cite{Leg07}.


==> introduction-old.tex <==
\section{Introduction}

($\omega$-)Regular model-checking
\cite{KMMPS97,BJNT00,DLS02,AJNdo03,BLW03,BLW04a,BHV04,Leg07} is the
name of a family of techniques in which states are represented by
words, sets of states by finite automata on these objects, and
transitions by finite automata operating on pairs of state encodings,
i.e. finite-state transducers. In this context, the problem of
computing the set of reachable states of a system can be reduced to
the one of computing the iterative closure of the finite-state
transducer representing its transition relation. Given the
expressiveness of the framework these acceleration techniques cannot
be perfectly general and exact but, in many meaningful cases, they are
able to compute a regular representation (or approximation) of the
reachable states of infinite-state systems. However, computing
reachable states is not quite model-checking. For reachability
properties model checking can be reduced to a state reachability
problem, but for properties that include a linear-time temporal
component~\cite{Pnu77,LPZ85,Var88,GO03}, the best that can be
done is to reduce the linear-time model-checking problem to emptiness
of a B\"uchi automaton~\cite{VW86}, which means checking for repeated
reachability rather than reachability.

In this paper, we consider the specification and the verification of
linear temporal properties in the ($\omega$-)regular model checking
framework. The main objective of the paper is to provide a general
specification framework and generic analysis techniques covering
various classes of systems that can be encoded in the
($\omega$-)regular model checking framework{\footnote{In the rest of
the paper, we use ``($\omega$-)regular model checking'' to denote
either ``regular model checking'' or ``$\omega-$regular model
checking'', depending on whether states are encoded by finite or infinite
words.}}. For those systems, whose states are represented by finite
(resp. infinite) words, an execution is an infinite sequence of such
words. To define a temporal property of such an execution, one has the
choice between moving within a state (horizontally) or between states
(vertically). One thus naturally thinks of a two-dimensional logic to
describe properties of such execution. However, rather than focusing
on the fine points of a logic for defining properties, we have chosen
to concentrate on the computational aspects of verification, and use
finite (or infinite) word automata as a basis for defining temporal
properties. On the executions we are considering, finite automata move
either horizontally or vertically and clearly both are needed to
define meaningful properties. One could consider arbitrary alternation
between both directions, but in practice, one alternation is
sufficient. We thus limited our study to horizontal properties defined
in terms of vertical ones, which only makes sense for parametric
systems, i.e.  systems that are the result of the parallel composition
of an arbitrary number of identical finite-state processes, in which a
vertical slice corresponds to the execution of one process of the
system; as well as to vertical properties defined in terms of
horizontal ones, which makes sense for any ($\omega$)-regular
system. For both of these cases, we fully worked out how to augment
the transducer representing the system transitions in order to obtain
a transducer encoding the B\"uchi automaton resulting from combining
the system with the property.

Once the transition relation of the B\"uchi automaton has been
obtained, checking the automaton for nonemptiness is done by computing
the iterative closure of this relation, finding nontrivial cycles
between states, and finally checking for the reachability of states
appearing in such cycles. When dealing with systems where the number
of successors of each state is bounded, an accepting exectution of the
B\"uchi automaton will always contain the same state twice and hence
an identifiable cycle. However, when dealing with states whose length
can grow or that are infinite, there might very well be an accepting
computation of the B\"uchi automaton in which the same state never
appears twice.

To cope with this, we look for states that are not necessarily
identical, but such that one entails the other in the sense that
any execution possible from one is also possible from the other. The
exact notion of entailment we use is simulation.  For that, we compute
symbolically the greatest simulation relation on the states of
the system.

The nice twist is that the state of the symbolic representation of the
simulation relation is, in fact, the computation of the limit of a
sequence of finite-state transducers, for which the acceleration
techniques introduced in \cite{BLW03,BLW04a,Leg07} can also be
used. However, there are also several cases where this computation
converges after a finite number of steps, which has the added
advantage of guaranteeing that the induced simulation equivalence
relation partitions the set of configuration in a finite number of
classes, and hence that existing accepting computations will
necessarily be found, which might not be the case when the number of
simulation equivalence classes is infinite.\\
\newline
{\bf Structure of the paper.}  The paper is divided as follows. In
Section \ref{automata}, we recall the elementary definitions on
automata theory that will be used throughout the rest of the
paper. Section \ref{paper-model} present the ($\omega$-)regular model
checking framework. In Section \ref{liveness-observations}, we
introduce some definitions and recall elementary properties of
($\omega$-)regular systems. 
In Sections \ref{temporal-rmc1} and
\ref{last-thesis}, we introduce ($\omega$-)global system properties
that can be verified on any system that can be represented in the
($\omega$-)regular model checking framework. In Section
\ref{temporal-rmc2}, the definition of global system properties is
particularized to the case of parametric systems. In section
\ref{bool-liveness}, Boolean combinations of properties of different
types are considered. Section \ref{tree} discusses the extension of
the framework to tree regular model checking, where sets of states are
represented by tree automata. Finally, Sections \ref{related}
concludes the paper with a comparison with other work on the same
topic.


==> tree.tex <==
\section{A Brief Note on the Extension to Tree Regular Model Checking}
\label{tree}

There are many interesting infinite-state systems whose sets of
reachable states cannot be represented by regular sets of words. This
is either because the behavior of the system cannot be captured by a
regular representation \cite{FP01}, or because the topology of the
system is not suited to be described with a word-based
representation. A solution to the latter problem is to extend the
applicability of the ($\omega$-)regular model checking approach beyond
words. 

As an example, to verify systems which operate on {\em tree-like
  architectures}, such as the percolate protocol \cite{KMMPS97} or the
tree-arbiter protocol \cite{ABHQR97}, one can work with the {\it tree
  regular model checking} approach ~\cite{KMMPS97,AJMd02,BT02}. In
tree regular model checking, states are represented by trees, sets of
states by tree automata, and transitions by tree automata operating on
pairs of trees, {\emph{i.e.}} tree transducers.

Parametric systems are encoded in tree regular model checking
framework by representing each of their global states as a tree whose
nodes are linked to local states. It is fairly easy to see that all
the definitions and constructions introduced in Sections
\ref{temporal-rmc1} and \ref{temporal-rmc2} extend to
trees. Consequently, verifying local-oriented and global system
properties of tree parametric systems reduce to computing the
transitive closure of a tree transducer. This problem is undecidable,
but partial solutions have been provided in
\cite{AJMd02,BT02,ALRd05,ALRd06}.

When considering non locally-finite systems that are encoded in the
tree regular model checking framework, one can again work with a
simulation relation. This simulation can be over approximated with
techniques that can compute an extrapolation of the limit of an
infinite sequence of tree automata\,\cite{BT02,Tou03}.





